MFDNet: Multi-Frequency Deflare Network for Efficient Nighttime Flare Removal

When light is scattered or reflected accidentally in the lens, flare artifacts may appear in the captured photos, affecting the photos' visual quality. The main challenge in flare removal is to eliminate various flare artifacts while preserving the original content of the image. To address this challenge, we propose a lightweight Multi-Frequency Deflare Network (MFDNet) based on the Laplacian Pyramid. Our network decomposes the flare-corrupted image into low and high-frequency bands, effectively separating the illumination and content information in the image. The low-frequency part typically contains illumination information, while the high-frequency part contains detailed content information. So our MFDNet consists of two main modules: the Low-Frequency Flare Perception Module (LFFPM) to remove flare in the low-frequency part and the Hierarchical Fusion Reconstruction Module (HFRM) to reconstruct the flare-free image. Specifically, to perceive flare from a global perspective while retaining detailed information for image restoration, LFFPM utilizes Transformer to extract global information while utilizing a convolutional neural network to capture detailed local features. Then HFRM gradually fuses the outputs of LFFPM with the high-frequency component of the image through feature aggregation. Moreover, our MFDNet can reduce the computational cost by processing in multiple frequency bands instead of directly removing the flare on the input image. Experimental results demonstrate that our approach outperforms state-of-the-art methods in removing nighttime flare on real-world and synthetic images from the Flare7K dataset. Furthermore, the computational complexity of our model is remarkably low.

==> tabletex/table1.tex <==
\begin{table*}[ht]
\begin{center}
% \caption{\small \small \underline{\textbf{Real image denoising}} on SIDD~\cite{sidd} and DND~\cite{dnd} datasets. \textcolor{red}{$\ast$} denotes methods using additional training data. Our \xnet is trained only on the SIDD images and directly tested on DND. Among competing approaches, only \xnet surpasses $40$~dB PSNR.}
\caption{Quantitative comparison on Flare7K real-world and synthetic datasets in terms of PSNR, SSIM, LPIPS. The best results are highlighted in bold.}
\adjustbox{width=\linewidth}{
\begin{tabular}{c c| c c c c c c c c c c }
\toprule[0.15em]
\multicolumn{2}{c|}{\multirow{2}{*}{Dataset$\backslash$Method}} & {\multirow{2}{*}{Input}}& Zhang  & Sharma & Wu   & Dai  & HINet  & MPRNet & Restormer &Uformer & \textbf{MFDNet} \\
 & & &\cite{zhang2020nighttime} & \cite{sharma2021nighttime} & \cite{wu2021train} & \cite{dai2022flare7k} & \cite{chen2021hinet} & \cite{zamir2021multi} &  \cite{zamir2022restormer}	 & \cite{wang2022uformer} &  (Ours)  \\
\midrule[0.15em]
~ & PSNR~$\uparrow$ &  22.56& 21.02 &  20.49 & 24.61  &  26.11  &  26.74  & 26.14  & 26.28  & 26.60 & \textbf{26.98} \\
Real-world & SSIM~$\uparrow$ & 0.857& 0.784 &  0.826 & 0.871  &  0.879  &  0.882  & 0.878  & 0.883  & 0.892 & \textbf{0.895}\\
  & LPIPS~$\downarrow$ & 0.078& 0.174 &  0.112 & 0.060  &  0.055  &  \textbf{0.048}  & 0.050  & 0.054  & 0.051 & 0.051 \\
\midrule[0.1em]
~ & PSNR~$\uparrow$ & 22.77& 21.04 &  20.01 & 27.88  &  29.07  &  29.97  & 29.87  & 29.45  & 30.13 & \textbf{30.79} \\
Synthetic & SSIM~$\uparrow$ & 0.921& 0.841 &  0.865 & 0.952  &  0.958  &  0.959  & 0.959  & 0.950  & 0.965 & \textbf{0.966} \\
  & LPIPS~$\downarrow$ & 0.060& 0.136 &  0.111 & 0.031  &  0.022  &  0.021 & 0.020  & 0.025  & 0.020 & \textbf{0.019}  \\
\bottomrule[0.15em]
\end{tabular}
}
%\caption{Comparison results on Flare7K dataset in terms of PSNR, SSIM, LPIPS.}
\label{table:overall}
\end{center}
\end{table*}

==> tabletex/table2.tex <==
% \begin{table*}[!ht]
% \begin{center}
% \adjustbox{width=\linewidth}{
% \begin{tabular}{c | c c c  | c c c  | c c c  | c c c  | c c c  }
% \toprule[0.15em]
% %\rowcolor{color3} 
%    & \multicolumn{3}{c|}{\textbf{512$\times$512}} & \multicolumn{3}{c|}{\textbf{1024$\times$1024}} & \multicolumn{3}{c|}{\textbf{1080p}} & \multicolumn{3}{c|}{\textbf{2K}} & \multicolumn{3}{c}{\textbf{4K}} \\
% \cline{2-16}
% %\rowcolor{color3} 
%    Method  &GMACs & Params& Time~&GMACs& Params& Time ~ &GMACs & Params& Time~ &GMACs & Params& Time~&GMACs & Params& Time~  \\
%    ~&(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~   \\
% \midrule[0.15em]
% Dai~\cite{dai2022flare7k}  & 261.90 & 34.53 & 0.052 & 1047.61 & 34.53 & 0.195 & {$\ast$}&{$\ast$}&{$\ast$}&3682.99 & 34.53 & 0.686 & {-}&{-}&{-} \\
% HINet~\cite{chen2021hinet} & 682.86 & 88.67 & 0.119 & 2731.43 & 88.67 & 0.448 & {$\ast$}&{$\ast$}&{$\ast$}& {-}&{-}&{-} & {-}&{-}&{-} \\
% MPRNet~\cite{zamir2021multi}& 274.97 & \textbf{1.93} & 0.101 & 1099.87 & \textbf{1.93} & 0.377 & 2175.04&\textbf{1.93}&0.760&{-}&{-}&{-} & {-}&{-}&{-}  \\
% Restormer~\cite{zamir2022restormer}& 57.61 & 2.98 & 0.106 & 230.46 & 2.98 & 0.394 & 455.74&2.98&0.771&{-}&{-}&{-} & {-}&{-}&{-} \\
% % KPAC$_S$~\cite{son2021single_kpac} & \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  & 25.24 & 0.845 & ???  & 0.225\\
% Uformer~\cite{wang2022uformer} & 160.09 & 20.43 & 0.137 & 640.35 & 20.43 & 0.536 &{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}&{$\ast$}\\

% \textbf{MFDNet (ours)} &\textbf{18.25}  & 6.32&\textbf{0.034} & \textbf{73.01} & 6.32&\textbf{0.075}  & \textbf{144.53}  & 6.32&\textbf{0.153} & \textbf{256.66}  & \textbf{6.32}&\textbf{0.301}  & \textbf{578.12}  & \textbf{6.32}  & \textbf{0.783}   \\
% \bottomrule[0.15em]
% \end{tabular}
% }
% \caption{Comparison of the computational cost and time consumption.}  
% \label{table:efficiency}
% \end{center}
% \end{table*}

\begin{table*}[!ht]
\begin{center}
\caption{Comparison of the computational cost and time consumption on images from $512\times512$ resolution to 4K resolution. 'N.A.' denotes that the method cannot handle the input image of this size, and 'OOM' means that the method causes the out-of-memory issue for this specific resolution. The best results are highlighted in bold.} 
\adjustbox{width=\linewidth}{
\begin{tabular}{c | c c c  | c c c  | c c c  | c c c  | c c c  }
\toprule[0.15em]
%\rowcolor{color3} 
   & \multicolumn{3}{c|}{\textbf{512$\times$512}} & \multicolumn{3}{c|}{\textbf{1024$\times$1024}} & \multicolumn{3}{c|}{\textbf{1080p}} & \multicolumn{3}{c|}{\textbf{2K}} & \multicolumn{3}{c}{\textbf{4K}} \\
\cline{2-16}
%\rowcolor{color3} 
   Method  &GMACs & Params& Time~&GMACs& Params& Time ~ &GMACs & Params& Time~ &GMACs & Params& Time~&GMACs & Params& Time~  \\
   ~&(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~ &(G)~ & (M)~& (s)~   \\
\midrule[0.15em]
Dai~\cite{dai2022flare7k}  & 261.90 & 34.53 & 0.052 & 1047.61 & 34.53 & 0.195 & N.A.&N.A.&N.A.&3682.99 & 34.53 & 0.686 & {OOM}&{OOM}&{OOM} \\
HINet~\cite{chen2021hinet} & 682.86 & 88.67 & 0.119 & 2731.43 & 88.67 & 0.448 & N.A.&N.A.&N.A.& {OOM}&{OOM}&{OOM} & {OOM}&{OOM}&{OOM} \\
MPRNet~\cite{zamir2021multi}& 274.97 & \textbf{1.93} & 0.101 & 1099.87 & \textbf{1.93} & 0.377 & 2175.04&\textbf{1.93}&0.760&{OOM}&{OOM}&{OOM} & {OOM}&{OOM}&{OOM}  \\
Restormer~\cite{zamir2022restormer}& 57.61 & 2.98 & 0.106 & 230.46 & 2.98 & 0.394 & 455.74&2.98&0.771&{OOM}&{OOM}&{OOM} & {OOM}&{OOM}&{OOM} \\
% KPAC$_S$~\cite{son2021single_kpac} & \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  & 25.24 & 0.845 & ???  & 0.225\\
Uformer~\cite{wang2022uformer} & 160.09 & 20.43 & 0.137 & 640.35 & 20.43 & 0.536 &N.A.&N.A.&N.A.&N.A.&N.A.&N.A.&N.A.&N.A.&N.A.\\

\textbf{MFDNet (ours)} &\textbf{18.25}  & 6.32&\textbf{0.034} & \textbf{73.01} & 6.32&\textbf{0.075}  & \textbf{144.53}  & 6.32&\textbf{0.153} & \textbf{256.66}  & \textbf{6.32}&\textbf{0.301}  & \textbf{578.12}  & \textbf{6.32}  & \textbf{0.783}   \\
\bottomrule[0.15em]
\end{tabular}
}
%\caption{Comparison of the computational cost and time consumption.}  
\label{table:efficiency}
\end{center}
\end{table*}


==> tabletex/table3.tex <==
\begin{table}[!htb]
\begin{center}
% \caption{\small \small \underline{\textbf{Real image denoising}} on SIDD~\cite{sidd} and DND~\cite{dnd} datasets. \textcolor{red}{$\ast$} denotes methods using additional training data. Our \xnet is trained only on the SIDD images and directly tested on DND. Among competing approaches, only \xnet surpasses $40$~dB PSNR.}
%\vspace{-2mm}
%\setlength{\tabcolsep}{7pt}
\caption{Ablation experiments of individual components in our MFDNet on Flare7K dataset.}
\adjustbox{width=\columnwidth}{
\begin{tabular}{c c| c c c c}
\toprule[0.15em]
\multicolumn{2}{c|}{Dataset$\backslash$Network} & w/o FETB+FRTB & w/o FECB+FDCB   & w/o FAB & MFDNet \\
% \textbf{Dataset} & & \cite{DnCNN} & \cite{BM3D} & \cite{CBDNet} & \cite{RIDNet} & \cite{kim2020aindnet} & \cite{VDN} &  \cite{chang2020sadnet}	 & \cite{yue2020danet} &  \cite{zamir2020cycleisp}  \\
\midrule[0.15em]
~ & PSNR~$\uparrow$ &  26.36 &  24.94  & 26.70  & \textbf{26.98} \\
Real-world  & SSIM~$\uparrow$&  0.890  &  0.872  &  0.894 & \textbf{0.895}\\
  & LPIPS~$\downarrow$   &  0.054  &  0.066 &  0.053  &  \textbf{0.051}\\
\midrule[0.1em]
~ & PSNR~$\uparrow$  &  30.32  &  25.95  & 30.61  & \textbf{30.79} \\
Synthetic  & SSIM~$\uparrow$ &  0.963  &  0.925  &  0.964 & \textbf{0.966} \\
  & LPIPS~$\downarrow$  &   0.021 &  0.046 &  0.021  & \textbf{0.019}  \\
\bottomrule[0.15em]
\end{tabular}
}
%\caption{Ablation experiments on Flare7K dataset.}
\label{table:ablation}
\end{center}
\end{table}
